Distances for Comparing Multisets and Sequences

Measuring the distance between data points is fundamental to many statistical techniques, such as dimension reduction or clustering algorithms. However, improvements in data collection technologies has led to a growing versatility of structured data for which standard distance measures are inapplicable. In this paper, we consider the problem of measuring the distance between sequences and multisets of points lying within a metric space, motivated by the analysis of an in-play football data set. Drawing on the wider literature, including that of time series analysis and optimal transport, we discuss various distances which are available in such an instance. For each distance, we state and prove theoretical properties, proposing possible extensions where they fail. Finally, via an example analysis of the in-play football data, we illustrate the usefulness of these distances in practice.

==> 4-simulations.tex <==
\section{Simulations}

\subsection{Ordered vs unordered distances}

\subsection{Comparing hypergraphs}

Let $\Hyp = \{e_1,\dots,e_M\}$ denote a hypergraph, where $e_i \in \mathcal{P}(\V)$ denote hyperedges, i.e. subsets of vertices. If $\G_\Hyp$ denote the (integer weighted) cooccurrence graph obtained from $\Hyp$, then one can imagine we may have
$$\G_\Hyp = \G_{\Hyp^\prime} $$
for $\Hyp \not=\Hyp^\prime$. In such situations, which might expect a distance between hypergraphs to do much better at distinguishing data points than graph distances between their aggregates. Here we look to construct a simulation showing this. 

I have fleshed out an approach which, given some $\Hyp$, will randomly sample a $\Hyp^\prime$ such that $\G_\Hyp = \G_{\Hyp^\prime}$. The idea is a sequential procedure which iteratively adds hyperedges to $\Hyp^\prime$, keeping track of edges in the occurrence graph $\G_{\Hyp^\prime}$, stopping when $\G_{\Hyp}=\G_{\Hyp^\prime}$. 

A possible simulation would thus be the following 
\begin{enumerate}
    \item Sample some hypergraph $\Hyp$ 
    \item Sample $\{\Hyp_k\}_{k=1}^K$ s.t. $\G_{\Hyp} = \G_{\Hyp_k}$ 
    \item For $k=1,\dots,K$ sample $n$ hypergraphs by perturbing $\Hyp_k$
    \item Compare metrics by 
    \begin{itemize}
        \item MDS plot of \textit{all} data with
        \item Ability to classify hypergraphs into one of the $K$ classes via k-nearest neighbours
    \end{itemize}
    focusing mainly on the difference between (i) distance between hypergraphs via our multiset distances (ii) distances between cooccurrence graphs (iii) crude distances between hypergraphs (e.g. hamming/jaccard) 
\end{enumerate}

Questions
\begin{itemize}
    \item Should we sample $\Hyp$ from some hypergraph model? E.g. \citep{ng2021hypergraph}
    \item How to perturb a hypergraph? How should we parameterise it? 
\end{itemize}


\subsection{Multi-layered graph random walk}

Here we consider trying to highlight analogous behaviour but for multisets of paths $\E = \{\I_i,\dots,\I_N\}$ where $\I_i = (x_{i1},\dots,x_{in_i})$ and $x_{ij} \in \V$. That is, we want to find some $\E^\prime \not=\E$ such that 
$$\G_\E = \G_{\E^\prime}.$$
An idea was inspired from a diagram in \cite{lambiotte2019}.



==> computation/matching_distance_via_ot.tex <==

To evaluate the matching distance requires optimising over all possible matchings of the two sets. One can, however, recast this problem in the light of Optimal Transport (OT) such that the output solution is guaranteed to be an optimal matching. Practically, this implies we can reuse the algorithm for calculating the Earth Mover's Distance (or Kantarovich distance). This not only simplifies the coding task, but also opens the door to use of open source code such as the Python Optimal Transport (POT) library. 

All we have to do is set up a suitable transportation problem, that is, one which is guaranteed to return the desired optimal matching. Key to this approach is a result seen in \cite{Peyre2019}. Before giving details some notation must be introduced. Imagine we have two \textit{histograms} $\mathbf{a}$ and $\mathbf{b}$, of size $n$ and $m$ respectively. That is, $\mathbf{a} \in \Delta_n$ and $\mathbf{b} \in \Delta_m$ where $$\Delta_r = \{(x_1,\dots, x_r) \, : \, \sum_{i=1}^r x_i = 1\}$$ is the $r$-dimensional simplex. Assume further that we have a cost matrix $(\mathbf{C}_{ij})_{i \in [n], j \in [m]}$, where $\mathbf{C}_{ij}$ is interpreted as the cost of transporting one unit of mass from location $i$ of $\mathbf{a}$ to location $j$ of $\mathbf{b}$. The key problem of optimal transport is solving the so-called Kantarovich problem 
\begin{align}
L_{\mathbf{C}}(\mathbf{a}, \mathbf{b}) = \min_{\mathbf{P} \in \mathbf{U}(\mathbf{a}, \mathbf{b})} \sum_{i\in [n], j \in [m]} \mathbf{P}_{ij}\mathbf{C}_{ij}, 
\label{eq:ot_lp}
\end{align}
where the cost of the optimal solution is taken as the distance between $\mathbf{a}$ and $\mathbf{b}$.
We also now define the notion of a \textit{permutation matrix}. For a permutation $\pi$ of $[n]$ we write the corresponding permutation matrix as the following
$$(\mathbf{P}_\pi)_{ij} = \begin{cases}
	1/n & \text{ if } \pi(i) = j \\
	0 & \text{ else}
\end{cases}$$ 
for $i,j \in [n]$. 
\begin{thm}
	(\cite{Peyre2019}, Proposition 2.1) If both histograms are uniform and of the same size, that is $$\mathbf{a} = \mathbf{b} = (1/n, \dots, 1/n) \in \Delta_n$$
	for some $n$, then, for a given cost matrix $\mathbf{C}$, the optimal solution $\mathbf{P}^*$ of $L_\mathbf{C}(\mathbf{a}, \mathbf{b})$ is a permutation matrix.  
\end{thm}

\begin{proof}
	 We here outline the argument given in \cite{Peyre2019}. Firstly, observing the feasible region $\mathbf{U}(\mathbf{a}, \mathbf{b})$ of the linear program (\ref{eq:ot_lp}) is a non-empty polyhedron, one can invoke a well-known result in linear programming to deduce the optimal solution of $L_\mathbf{C}(\mathbf{a}, \mathbf{b})$ will be reached at an extremal point of $\mathbf{U}(\mathbf{a}, \mathbf{b})$. The result then follows by invoking another result of \cite{Birkhoff1946}, which says the extremal points of $\mathbf{U}(\mathbf{a}, \mathbf{b})$ is equal to the set of permutation matrices.
\end{proof}

We now show that one can construct an OT problem which will lead to an optimal matching with regards to $d_M$ and $d_{M,\rho}$. There will be two cases 
\begin{enumerate}
	\item Guaranteed complete matching: this is for any case where only matchings including all elements of the smaller set can be optimal, e.g. this will be the case for $d_M$ and $d_{M, \rho}$ (when $\rho$ is an upper bound on the ground distance);
	\item General matching: this is for when any matching is potentially optimal, even one which matches no elements. 
\end{enumerate}
We separate these two cases since the former requires a smaller OT problem than the latter and will therefore be cheaper to compute. 

\subsubsection{Case 1: Guaranteed Complete Matching}

We will here adopt general notation. Assume that $X=\{x_1,\dots, x_n\}$ and $Y=\{y_1,\dots, y_m\}$ are two multisets of elements in some metric space $(\X, d)$. That is, $x,y \in \X$ for $x \in X$ and $y \in Y$, and $d(\cdot,\cdot)$ is a distance metric between elements of $\X$. 

Assume without loss of generality that $n \geq m$. The approach here is to essentially introduce $m-n$ new locations in the OT problem when can play the role of penalising unmatched elements. Let $\mathbf{C} \in \mathbb{R}_+^{n \times m}$ denote the pairwise distances between elements of $X$ and $Y$, that is, $\mathbf{C}_{ij} = d(x_i, y_j)$. Now, we construct a square matrix $\mathbf{C}^* \in \mathbb{R}_+^{n \times n}$ via 
\begin{equation}
	\begin{aligned}
		\mathbf{C}^* = [\mathbf{C} \,\,  \mathbf{E}]
	\end{aligned}
\end{equation}
where 
\begin{equation}
	\begin{aligned}
		\mathbf{E}_{ij} = \Omega(y_i)
	\end{aligned}
\end{equation}
with $\Omega(y)$ denoting the penalty term for any $y \in Y$ not being included in the matching. Note that this will depend on the matching distance one is considering, for example, in $d_M$ we have $\Omega(y) = d(\Lambda, y)$ whilst for $d_{M,\rho}$ we have $\Omega(y) = \rho/2$. Now, letting $\mathbf{a} = (1/n, \dots, 1/n) \in \Delta_n$ we take 

$$L_{\mathbf{C}^*}(\mathbf{a}, \mathbf{a}) =  \min_{\mathbf{P} \in \mathbf{U}(\mathbf{a}, \mathbf{a})} \sum_{i \in [n], j \in [n]}\mathbf{P}_{ij} \mathbf{C}_{ij}^*$$  

The justification for why this works is the following. 
\begin{itemize}
	\item Every \textit{complete} matching can be represented via a permutation matrix $\mathbf{P}$, where the extra entries of $\mathbf{C}^*$ allow one to capture the unmatched elements, or what we might see as elements being matched to the null element. Thus the set of permutation matrices is equal to the set of complete matchings;
	\item Furthermore, since we have a square cost matrix and uniform histograms the optimal solution is guaranteed to be a permutation matrix. Thus the optimal solution will be the optimal complete matching. And, provided for the given distance we know the optimal solution will be complete, this will be our desired optimal matching, from which one can evaluate the distance.
\end{itemize}

\subsubsection{Case 2: General Matching}


Justification in this case will be much the same 
\begin{itemize}
	\item Every matching can be represented via a permutation matrix, where this time the extra entries are required to capture cases such as all elements being left unmatched;
	\item The justification then follows as before.
\end{itemize}


==> distances/aggregates.tex <==
\subsection{Using Aggregates}

Though interaction network data has temporal information, a more obvious and simple way to measure distance is by first aggregating each observation. We could aggregate
\begin{itemize}
	\item Vertex counts;
	\item Edge counts/weighted graph;
	\item Motif counts;
	\item Single sequence (not partitioned into paths).
\end{itemize}

Following aggregation, one can then consider applying distance between the obtained objects. It should be noted that, though such distances might be metrics between the the aggregated objects, this map not being injective makes for induced measures not being genuine distance metrics between the original observations.

Some current ideas:
\begin{itemize}
		\item Vertex counts
	\begin{itemize}
		\item Hamming/Jaccard Distance;
		\item Earth Mover's Distance where ground distance, in this case the pairwise distance of vertices, are provided as input (obtained in pre-processing step);
	\end{itemize}
	\item Weighted graphs
	\begin{itemize}
		\item Hamming/Jaccard;
		\item Vertex centrality-based distances \cite{Donnat2018b};
		\item Wasserstein-based distances \cite{Maretic2019};
	\end{itemize}
	\item Motif counts
	\begin{itemize}
		\item Hamming/Jaccard;
	\end{itemize}
	\item Sequences
	\begin{itemize}
		\item Longest Common Subsequence/Subpath (\Cref{sec:dist_interactions});
		\item Normalsied versions;
	\end{itemize}

\end{itemize}
